Architectural improvements and technological enhancements for the APEnet+ interconnect system

The APEnet+ board delivers a point-to-point, low-latency, 3D torus network interface card. In this paper we describe the latest generation of APEnet NIC, APEnet v5, integrated in a PCIe Gen3 board based on a state-of-the-art, 28 nm Altera Stratix V FPGA. The NIC features a network architecture designed following the Remote DMA paradigm and tailored to tightly bind the computing power of modern GPUs to the communication fabric. For the APEnet v5 board we show characterizing figures as achieved bandwidth and BER obtained by exploiting new high performance ALTERA transceivers and PCIe Gen3 compliancy.

==> Makefile <==
DVIPS=dvips -t a4 
# -interaction=STRING     set interaction mode (STRING=batchmode/nonstopmode/
#                          scrollmode/errorstopmode)
#-halt-on-error
COMMON=-halt-on-error
#-interaction=nonstopmode
LATEX=latex -file-line-error $(COMMON)
PDFLATEX=pdflatex -file-line-error $(COMMON)
FILE=twepp14apenet
PDFS=$(FILE).pdf
TEXFILE=$(FILE).tex
AUXFILE=$(FILE).aux

pdf: $(PDFS)

.PHONY: pdf

%.pdf: %.tex
	$(PDFLATEX) $< && \
	bibtex $(AUXFILE) && \
	$(PDFLATEX) $< && \
	$(PDFLATEX) $<

%.dvi: %.tex
	$(LATEX) $<

%.ps: %.dvi
	$(DVIPS) -o $@ $<

paper.pdf: $(TEXFILE)

biblio:
	-latex -interaction=nonstopmode $(TEXFILE)
	bibtex $(FILE)

all: biblio pdf

clean:
	rm -f *.bbl *.aux *.log *.dvi *.toc *.err $(PDFS)


